Budget-optimal multi-robot layout design for box sorting

Robotic systems are routinely used in the logistics industry to enhance operational efficiency, but the design of robot workspaces remains a complex and manual task, which limits the system's flexibility to changing demands. This paper aims to automate robot workspace design by proposing a computational framework to generate a budget-minimizing layout by selectively placing stationary robots on a floor grid to sort packages from given input and output locations. Finding a good layout that minimizes the hardware budget while ensuring motion feasibility is a challenging combinatorial problem with nonconvex motion constraints. We propose a new optimization-based approach that models layout planning as a subgraph optimization problem subject to network flow constraints. Our core insight is to abstract away motion constraints from the layout optimization by precomputing a kinematic reachability graph and then extract the optimal layout on this ground graph. We validate the motion feasibility of our approach by proposing a simple task assignment and motion planning technique. We benchmark our algorithm on problems with various grid resolutions and number of outputs and show improvements in memory efficiency over a heuristic search algorithm.

==> root_graveyard.tex <==
With the task schedule specified, we refine the constraints stated in \cref{constr:ineq} to \cref{constr:initial} into a trajectory optimization formulation.
We discretize the trajectory into $n$ time steps and let $\x_{r,t}$ be the joint values of robot $r$ at time step $t$.
The joint angles are subjected to box constraints of the form $x^\mathrm{min}_r \leq \x_{r,t} \leq x^\mathrm{max}_r$ that correspond to the physical joint limit of the robot.
We use \(\mathbf{f}_{r}\ :\ \mathbb{R}^{d_i} \mapsto SE(3)\) for denoting the forward kinematic function that maps the joint state \(\mathbf{x}_{r}\) of robot \(r\) to an end effector pose in the world coordinate frame.
Let $\Phi^i$ and $\Psi^i$ be box $ i$'s initial and goal pose in the world coordinate frame corresponding to its input and output locations.

\subsubsection{Kinematic switch constraints} 
The pose of a box is constrained by the kinematic equations that are induced by the robot holding it.
When the scheduling function $s^i$ has a discontinuity, this set of constraints changes, and these moments are known as the kinematic switches.
Every time a robot arm \(r\) picks up box $i$ at time step \(t\), its end effector's pose should match the box's initial pose \(\Phi^i\):
\begin{equation}
    C_\mathrm{pick}:=\left\| \mathbf{f}_r(\mathbf{x}_{r, t}) 
    - \Phi^i \right\|
    = 0 
\end{equation}

Similarly, every time a robot arm places down a box:
\begin{equation}
    C_\mathrm{place}:=\left\| \mathbf{f}_r(\mathbf{x}_{r, t}) 
    - \Psi^i \right\|
    = 0 
\end{equation}

We introduce a function \(\textsc{Reverse}\ :\ SE(3) \mapsto SE(3)\) to reverse an end effector's axes for handover with another end effector. Then, the constraint for handover: 
\begin{equation}
    C_\mathrm{hand}:=\left\| \mathbf{f}_{r_1}(\mathbf{x}_{{r_1}, t}) 
    - \textsc{Reverse} \left[
    \mathbf{f}_{r_2}(\mathbf{x}_{{r_2}, t})  \right]\right\|
    = 0 
\end{equation}

Given a task schedule, we define three sets \(\textsc{Pick}\), \(\textsc{Place}\), \(\textsc{Hand}\) to record all picking/placing/handover events. 

% Then, the constraints for all picking-up events could be written as
% \begin{equation}
%     \mathbf{C}_{pick} := \left(C_{pick}, \forall \left(r, \Phi, t\right) \in \textsc{Pick}\right) = \mathbf{0}
% \end{equation}
% \begin{subequations}
%     \begin{alignat}{3}
%         &\mathbf{C}_{pick} &&:= \left(C_{pick}, \forall \left(r, \Phi, i\right) \in \textsc{Pick}\right) &&= \mathbf{0}
%         &\mathbf{C}_{pick} &&:= \left(C_{pick}, \forall \left(r, \Phi, i\right) \in \textsc{Pick}\right) &&= \mathbf{0}\\
%         &\mathbf{C}_{hand} &&:= \left(C_{hand} = 0, \forall \left(r_1, r_2, i\right) \in \textsc{Hand}\right) &&= \mathbf{0}
%     \end{alignat}
% \end{subequations}

% \subsubsection{Joint limit}
% We use \(\textsc{Up}_r\) and \(\textsc{Low}_r\) to denote the upper and lower bound for joint angles of robot \(r\in\mathcal{R}\). The joint limit constraints for robot \(r\) can be written as
% \begin{subequations}
%     \begin{alignat}{3}
%         &\mathbf{C}_{up,r}&&:=
%         \mathbf{x}_{r} - \textsc{Up}_r &&< \mathbf{0}\\
%         &\mathbf{C}_{low,r}&&:=
%         \mathbf{x}_{r} - \textsc{Low}_r &&> \mathbf{0}
%     \end{alignat}
% \end{subequations}

\subsubsection{Collision avoidance constraints}
We attach a series of spheres to the links of robot arms to approximate their collision meshes. 
Collision-free trajectories are ensured by imposing a collision avoidance constraint of the form:
\begin{equation}
    C_\mathrm{collision} := \textsc{Dist}(\mathcal{K}_a(\mathbf{x}), \mathcal{K}_b(\mathbf{x})) > 0, \forall a, b \in \mathcal{C}
\end{equation}
where $\mathcal{K}_a$ and $\mathcal{K}_b$ denote a pair of forward kinematic functions for collision spheres $a, b \in \mathcal{C}$ in the scene and $\textsc{Dist}$ computes the squared distance between spheres.

\subsubsection{Trajectory optimization}
By stacking all robot trajectories into $\x$, we can now write the trajectory optimization problem as:
% 
\begin{subequations}\label{eq:motion_trajectory}%
    \begin{alignat}{3}
        \min_{\mathbf{x}} &&\ \mathcal{O}\left(\mathbf{x}\right) \label{eq:objective}\\
        s.t. &&\ C_\mathrm{pick}&& = 0,\ &\forall \left(i, r, \Phi^i, t\right) \in \textsc{Pick}\\
        &&\ C_\mathrm{place}&& = 0,\ &\forall \left(i, r, \Psi^i, t\right) \in \textsc{Place}\\
        &&\ C_\mathrm{hand}&& = 0,\ &\forall \left(r_1, r_2, t\right) \in \textsc{Hand}\\
        % &&\ \mathbf{C}_{up,r}&& < \mathbf{0},\ &\forall r\in \mathcal{R}\\
        % &&\ \mathbf{C}_{low,r}&& > \mathbf{0},\ &\forall r\in \mathcal{R}\\
        &&\ C_\mathrm{collision}&& > 0,\ &\forall a,b\in\textsc{Collision}\\
        &&\ \x^{min}_r && \leq \x_{r,t} &\leq \x^{max}_r,\ \forall r\in \mathcal{R}
    \end{alignat}
\end{subequations}
where \(\mathcal{O}(\mathbf{x})\) is the objective function that penalizes joint velocities and accelerations of each robot:
\begin{equation}
    \mathcal{O}(\mathbf{x}) = \sum_{r\in\mathcal{R}}
    \left[ \beta_v \sum \|\dot{\mathbf{x}}_r\| + \beta_a \sum \|\ddot{\mathbf{x}}_r\|\right]
\end{equation}
where \(\beta_v, \beta_a \in \mathbb{R}\) are constant weights.

To solve the constrained non-convex optimization problem \ref{eq:motion_trajectory} numerically, we convert it to an unconstrained problem by applying quadratic and cubic penalty functions to the equality and inequality constraints respectively, and solve it using the Gauss-Newton method.

\paragraph{Modeling conveyor belts in motion planning}
We model a conveyor belt segment as a manipulator with multiple fictitious end effectors fixed to a prismatic joint. 
Each end effector of the conveyor belt can hold one box on the belt.
The state vector of a belt $r$ includes the prismatic joint's value $x^p_{r,t}$ and the grasp variables $x_{r,i}$ that describe the relative transformation between the end effector holding box $i$ and the prismatic joint.
% (\cref{fig:conveyor_belt_mp}).
Since the boxes cannot slide once placed on the belt, the grasp variables are time-independent and are shared across all time steps $t$.
We assume that the conveyor belt maintains a constant speed, so $x^p_{r,i}$ is affine to the time step.
% and requires its own forward kinematics functions \(\mathbf{f}_{r,i}(\mathbf{x}_{r,t}), i\in\{1, 2, \ldots, N\}\) to express the grasping relationship.

% \begin{figure}[thpb]
%     \centering
%     \includegraphics[width = 1.0\columnwidth]{img/conveyor_belt.png}
%     \caption{Illustration of the state space of a conveyor belt with three fictitious end effectors. $x_{r,t}$ is the prismatic joint value, and $x_{r,i}$ is the grasp transformation between end effector $i$ and the prismatic joint.}
%     \label{fig:conveyor_belt_mp}
% \end{figure}

During the time steps when a belt is handling a box, we add the following constraints to the trajectory optimization \cref{eq:motion_trajectory} to ensure that the end effector holding the box \(i\) stays on the belt, not floating in the space along its extended line:
% 
\begin{equation}
    -\frac{1}{2} L_r < \mathbf{f}_{r,i}(x^p_{r,t}, x_{r,i}).x < \frac{1}{2} L_r, \ \forall t, \ s.t. \ s^i(t) = r
\end{equation}
where \(t\) is the time step that the box \(i\) should stay on the belt, \(\mathbf{f}_{r,i}\) is the forward kinematics function of end effector \(i\) in the base frame of the conveyor belt, and \(L_r\) is the belt length.

% Another characteristic of the conveyor belt is that each end effector remains static to the other during execution since boxes cannot be actuated separately and cannot slide when they are on the same belt. Thus, the entries corresponding to the relative pose of the end effector to the belt in the state vector \(\mathbf{x}_{r,t}\) keep the same value for all \(t\in T\), which means they are time-invariant. Each state \(\mathbf{x}_{r,t}\) of a conveyor belt could be divided into two parts: the time-variant part \(\mathbf{x}_{r,t}^{act}\) and the time-invariant part \(\mathbf{x}_{r}^{static}\). While stacking the state vectors \(\mathbf{x}_{r,t}\) of all time steps \(t\in T\) of a conveyor belt, we only need to store the time-invariant part \(\mathbf{x}_{r}^{static}\) once. We can use this property to simplify the motion planning problem by reducing the number of variables and constraints. 

% We assume that the speed of the conveyor belt does not change during execution, which means the joint value for the belt movement is affine to the time step. Thus, only two variables of two different time steps are needed to compute the belt movement during the whole execution \(i\in T\). Similarly to the presence of a static part of the state vector, there is also an affine part in the state vector of a conveyor belt, which could simplify the motion planning problem further.
